Near Real-Time Data-Driven Control of Virtual Reality Traffic in Open Radio Access Network

In mobile networks, Open Radio Access Network (ORAN) provides a framework for implementing network slicing that interacts with the resources at the lower layers. Both monitoring and Radio Access Network (RAN) control is feasible for both 4G and 5G systems. In this work, we consider how data-driven resource allocation in a 4G context can enable adaptive slice allocation to steer the experienced latency of Virtual Reality (VR) traffic towards a requested latency. We develop an xApp for the near real-time RAN Intelligent Controller (RIC) that embeds a heuristic algorithm for latency control, aiming to: (1) maintain latency of a VR stream around a requested value; and (2) improve the available RAN allocation to offer higher bit rate to another user. We have experimentally demonstrated the proposed approach in an ORAN testbed. Our results show that the data-driven approach can dynamically follow the variation of the traffic load while satisfying the required latency. This results in 15.8% more resources to secondary users than a latency-equivalent static allocation.

==> 0.5abstract.tex <==
%data-driven, ORAN, VR, heterogeneous service requirements, latency, network slicing
%With the rising interest in 5G and network slicing towards providing heterogeneous service requirements for multiple users at once, an issue becomes how to do so in an efficient way that enables co-existence between the users and services. ORAN proposes an architecture enabling control and monitoring tools of the \gls{ran} realized through xApps utilizing the \gls{ric}. In this work we leverage the ORAN \gls{ric} for \gls{ran}-slicing to make a data-driven resource allocation. The purpose being to keep the latency of video frames sent to a user around a requested amount, while not over allocating resources to enable other users a decent experience as well. We evaluate this on a physical live test bed where the xApp monitors \gls{ran} statistics, infers on the latency the user experiences, and allocates accordingly. 



Network slicing is one of the newer paradigms envisioned to improve the heterogeneous requirements of different services and applications. While it is primarily envisioned for 5G, OpenRAN establishes a framework, where monitoring and \gls{ran} control is feasible for both 4G and 5G. xApps are proposed as applications executing on the near real-time \gls{ric} to consume data and execute control of the \gls{ran} with the potential of integrated intelligence in the network. In this work we consider how data-driven resource allocation in a 4G context can be used to update slice allocation to steer the experienced latency of \gls{vr} traffic towards a requested latency. As a first step this is done with a heuristic approach, but which can be further enriched in the future.
The experiments are evaluated physically on a test bed, where we maintain a latency around the request with the data driven allocation while allowing the \gls{ran} resources to be better shared by another user leading to higher bit rate for them compared to static and no slicing.
The relevance of the data-driven approach is especially derived from the variation of the required traffic load, and while static allocations may be able to give similar performance it will likely be unknown in advance what static allocation is actually required to have the average latency.


